An approximate control variates approach to multifidelity distribution estimation

Forward simulation-based uncertainty quantification that studies the distribution of quantities of interest (QoI) is a crucial component for computationally robust engineering design and prediction. There is a large body of literature devoted to accurately assessing statistics of QoIs, and in particular, multilevel or multifidelity approaches are known to be effective, leveraging cost-accuracy tradeoffs between a given ensemble of models. However, effective algorithms that can estimate the full distribution of QoIs are still under active development. In this paper, we introduce a general multifidelity framework for estimating the cumulative distribution function (CDF) of a vector-valued QoI associated with a high-fidelity model under a budget constraint. Given a family of appropriate control variates obtained from lower-fidelity surrogates, our framework involves identifying the most cost-effective model subset and then using it to build an approximate control variates estimator for the target CDF. We instantiate the framework by constructing a family of control variates using intermediate linear approximators and rigorously analyze the corresponding algorithm. Our analysis reveals that the resulting CDF estimator is uniformly consistent and asymptotically optimal as the budget tends to infinity, with only mild moment and regularity assumptions on the joint distribution of QoIs. The approach provides a robust multifidelity CDF estimator that is adaptive to the available budget, does not require \textit{a priori} knowledge of cross-model statistics or model hierarchy, and applies to multiple dimensions. We demonstrate the efficiency and robustness of the approach using test examples of parametric PDEs and stochastic differential equations including both academic instances and more challenging engineering problems.

==> tmp_ex_article_header.tex <==
\title{An approximate control variates approach to multifidelity distribution estimation\thanks{Submitted to the editors on \today.
\funding{RH is partially supported by the Hong Kong Research Grants Council (grant no. 14301821) and Start-up Fund for New Recruits, The Hong Kong Polytechnic University.
AN is partially supported by NSF DMS-1848508 and AFOSR FA9550-20-1-0338.
BK and DL are supported by the Ministry of Trade, Industry and Energy (MOTIE) and the Korea Institute for Advancement
of Technology (KIAT) through the International Cooperative R\&D program (grant no. P0019804, Digital twin based intelligent unmanned facility inspection solutions).
The views expressed in this article do not necessarily represent the views of Wells Fargo.}}}

\author{
Ruijian Han\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University}
\and Boris Kramer\thanks{Department of Mechanical and Aerospace Engineering, University of California San Diego}
\and Dongjin Lee\footnotemark[3]
\and Akil Narayan\thanks{Scientific Computing and Imaging Institute, and Department of Mathematics, University of Utah}
\and Yiming Xu\thanks{Corporate Model Risk, Wells Fargo
  (\email{yiming2358@gmail.com}).}}

% Custom SIAM macro to insert headers
\headers{Multifidelity distribution estimation}{R. Han and B. Kramer and D. Lee and A. Narayan and Y. Xu}


==> tmp_ex_supplement_header.tex <==
\title{An approximate control variates approach to multifidelity distribution estimation\thanks{Submitted to the editors on \today.
\funding{RH is partially supported by the Hong Kong Research Grants Council (grant no. 14301821) and Start-up Fund for New Recruits, The Hong Kong Polytechnic University.
AN is partially supported by NSF DMS-1848508 and AFOSR FA9550-20-1-0338.
BK and DL are supported by the Ministry of Trade, Industry and Energy (MOTIE) and the Korea Institute for Advancement
of Technology (KIAT) through the International Cooperative R\&D program (grant no. P0019804, Digital twin based intelligent unmanned facility inspection solutions).
The views expressed in this article do not necessarily represent the views of Wells Fargo.}}}

\author{
Ruijian Han\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University}
\and Boris Kramer\thanks{Department of Mechanical and Aerospace Engineering, University of California San Diego}
\and Dongjin Lee\footnotemark[3]
\and Akil Narayan\thanks{Scientific Computing and Imaging Institute, and Department of Mathematics, University of Utah}
\and Yiming Xu\thanks{Corporate Model Risk, Wells Fargo
  (\email{yiming2358@gmail.com}).}}

% Custom SIAM macro to insert headers
\headers{Multifidelity distribution estimation}{R. Han and B. Kramer and D. Lee and A. Narayan and Y. Xu}

